A transformer boosted UNet for smoke segmentation in complex backgrounds in multispectral LandSat imagery

Many studies have been done to detect smokes from satellite imagery. However, these prior methods are not still effective in detecting various smokes in complex backgrounds. Smokes present challenges in detection due to variations in density, color, lighting, and backgrounds such as clouds, haze, and/or mist, as well as the contextual nature of thin smoke. This paper addresses these challenges by proposing a new segmentation model called VTrUNet which consists of a virtual band construction module to capture spectral patterns and a transformer boosted UNet to capture long range contextual features. The model takes imagery of six bands: red, green, blue, near infrared, and two shortwave infrared bands as input. To show the advantages of the proposed model, the paper presents extensive results for various possible model architectures improving UNet and draws interesting conclusions including that adding more modules to a model does not always lead to a better performance. The paper also compares the proposed model with very recently proposed and related models for smoke segmentation and shows that the proposed model performs the best and makes significant improvements on prediction performances

==> pix-mod-Article-front.tex <==
% !Tex root = pixmodel.tex

%\documentclass[preprint]{elsarticle} 
% detailed Elsevier front matter is in JXnotes\use-latex.tex.

 \title{A transformer boosted UNet for smoke segmentation  in complex backgrounds in multispectral Landsat imagery}
\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao \\
UniSA STEM, University of South Australia \\
\{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}@unisa.edu.au}

\maketitle

 \begin{abstract}
 Many studies have been done to detect smokes from satellite imagery. However, these prior methods are not still effective in detecting various smokes in complex backgrounds. Smokes present challenges in detection due to variations in density, color, lighting, and backgrounds such as clouds, haze, and/or mist. This paper addresses these challenges by proposing a new segmentation model called  VTrUNet which consists of a feature construction module and a transformer boosted UNet. The model takes imagery of six bands: red, green, blue, near infrared, and two shortwave infrared bands as input. To show the advantages of the proposed model, the paper presents extensive results for various possible model architectures improving UNet. The paper also compares the proposed model with very recently proposed and related models for smoke segmentation and shows that the proposed model performs the best and makes significant improvements on prediction performances. 
\end{abstract}

{\bf Keywords: } 
 smoke detection, satellite imagery, self attention, transformer, evaluation metrics




==> pix-mod-Elsevier-front.tex <==
% !Tex root = pixmodel.tex
%\documentclass[preprint]{elsarticle} 

 \journal{International Journal of Applied Earth Observation and Geoinformation}

 \begin{frontmatter}
 \title{VTrUNet for smoke segmentation  in complex backgrounds from satellite imagery of six bands}
\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao \\
UniSA STEM, University of South Australia \\
\{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}@unisa.edu.au}

 \begin{abstract}
 Many studies have been done to detect smokes from satellite imagery. However, these prior methods are not still effective in detecting various smokes in complex backgrounds. Smokes present challenges in detection due to variations in density, color, lighting, and backgrounds such as clouds, haze, and/or mist and the contextual nature in detection. This paper addresses these challenges by proposing a new segmentation model called  VTrUNet which consists of a feature construction module and a transformer boosted UNet. The model takes imagery of six bands: red, green, blue, near infrared, and two shortwave infrared bands as input. To show the advantages of the proposed model, the paper presents extensive results for various possible model architectures improving UNet. The paper also compares the proposed model with very recently proposed and related models for smoke segmentation and shows that the proposed model performs the best and makes significant improvements on prediction performances. 
\end{abstract}

\begin{keyword} 
 smoke detection, satellite imagery, self attention, transformer, evaluation metrics
\end{keyword}

 \end{frontmatter}
%\maketitle



==> pix-mod-IEEE-front.tex <==
% !Tex root = pixmodel.tex

\title{A transformer boosted UNet for smoke segmentation from satellite imagery of six bands}

%\title{VTrUNet detecting detecting relative thin smoke pixels}
\title{VTrUNet for smoke segmentation  in complex backgrounds from satellite imagery of six bands}
%\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao\\
%   \IEEEauthorblockA{\{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}%@unisa.edu.au}\\
%    \IEEEauthorblockA{UniSA STEM, University of South Australia }
%}
\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao 
\thanks{  All authors are from UniSA STEM, University of South Australia. Their emails are \{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}@unisa.edu.au}
}

% The paper headers
%\markboth{IEEE Transaction on Geoscience and Remote Sensing}
%{Shell \MakeLowercase{\textit{Liu et al.}}: Relative Smoke Detection}

%\IEEEpubid{0000--0000/00\$00.00~\copyright~2021 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.

\maketitle



\begin{abstract}
Many studies have been done to detect smokes from satellite imagery. However, these prior methods are not still effective in detecting various smokes in complex backgrounds. Smokes present challenges in detection due to variations in density, color, lighting, and backgrounds such as clouds, haze, and/or mist. This paper addresses these challenges by proposing a new segmentation model called  VTrUNet which consists of a feature construction module and a transformer boosted UNet. The model takes imagery of six bands: red, green, blue, near infrared, and two shortwave infrared bands as input. To show the advantages of the proposed model, the paper presents extensive results for various possible model architectures improving UNet. The paper also compares the proposed model with very recently proposed and related models for smoke segmentation and shows that the proposed model performs the best and makes significant improvements on prediction performances. 
\end{abstract}

\begin{IEEEkeywords}
smoke detection, satellite imagery, self attention, transformer, evaluation metrics
\end{IEEEkeywords}

\iffalse % carry on examples
\newcommand{\jxpara}[1]{\vspace{.5ex} \noindent {\bf #1}}%bf newenv
\newenvironment{jxproof}{{{\bf Proof }\begin{itshape}}{\end{itshape}$\Box$}}
\begin{itemize} \itemsep=0em \topsep=0em \parskip=0cm \partopsep=0cm \parsep=0cm
 \item   Item 1 content  
 \end{itemize}
\begin{align}
  fp(c) = \frac{\hat{c} }{\tilde{o}} \qquad  \quad \label{eq:pr-re-fpr}
\end{align}
\begin{figure}[h]  \begin{center}
\includegraphics[scale=0.9]{score-func.pdf}
\caption{\label{fig:score-func}   Diagram for   }
\end{center}	
\end{figure}
\begin{table} %https://www.overleaf.com/learn/latex/Tables
\begin{tabular}{ |c|c|c| }\hline
a & b & c \\ \hline
\end{tabular}
\end{table}
\fi

==> pix-mod-Springer-front.tex <==


\title{VTrUNet for smoke segmentation from satellite imagery of six bands}

%\title{VTrUNet detecting detecting relative thin smoke pixels}
\title{VTrUNet for smoke segmentation  in complex backgrounds from satellite imagery of six bands}
%\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao\\
%   \IEEEauthorblockA{\{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}%@unisa.edu.au}\\
%    \IEEEauthorblockA{UniSA STEM, University of South Australia }
%}
\author{Jixue Liu,  Jiuyong Li,  Stefan Peters, Liang Zhao 
\thanks{  All authors are from UniSA STEM, University of South Australia. Their emails are \{jixue.liu, jiuyong.li, stefan.peters, liang.zhao\}@unisa.edu.au}
}

% The paper headers
%\markboth{IEEE Transaction on Geoscience and Remote Sensing}
%{Shell \MakeLowercase{\textit{Liu et al.}}: Relative Smoke Detection}

%\IEEEpubid{0000--0000/00\$00.00~\copyright~2021 IEEE}
% Remember, if you use this you must call \IEEEpubidadjcol in the second
% column for its text to clear the IEEEpubid mark.

\maketitle



\begin{abstract}
Many studies have been done to detect smokes from satellite imagery. However, these prior methods are not still effective in detecting various smokes in complex backgrounds. Smokes present challenges in detection due to variations in density, color, lighting, and backgrounds such as clouds, haze, and/or mist. This paper addresses these challenges by proposing a new segmentation model called  VTrUNet which consists of a feature construction module and a transformer boosted UNet. The model takes imagery of six bands: red, green, blue, near infrared, and two shortwave infrared bands as input. To show the advantages of the proposed model, the paper presents extensive results for various possible model architectures improving UNet. The paper also compares the proposed model with very recently proposed and related models for smoke segmentation and shows that the proposed model performs the best and makes significant improvements on prediction performances. 
\end{abstract}

\begin{IEEEkeywords}
smoke detection, satellite imagery, self attention, transformer, evaluation metrics
\end{IEEEkeywords}

\iffalse % carry on examples
\newcommand{\jxpara}[1]{\vspace{.5ex} \noindent {\bf #1}}%bf newenv
\newenvironment{jxproof}{{{\bf Proof }\begin{itshape}}{\end{itshape}$\Box$}}
\begin{itemize} \itemsep=0em \topsep=0em \parskip=0cm \partopsep=0cm \parsep=0cm
 \item   Item 1 content  
 \end{itemize}
\begin{align}
  fp(c) = \frac{\hat{c} }{\tilde{o}} \qquad  \quad \label{eq:pr-re-fpr}
\end{align}
\begin{figure}[h]  \begin{center}
\includegraphics[scale=0.9]{score-func.pdf}
\caption{\label{fig:score-func}   Diagram for   }
\end{center}	
\end{figure}
\begin{table} %https://www.overleaf.com/learn/latex/Tables
\begin{tabular}{ |c|c|c| }\hline
a & b & c \\ \hline
\end{tabular}
\end{table}
\fi
